Alpha-GPT 2.0: Human-in-the-Loop AI for Quantitative Investment

Recently, we introduced a new paradigm for alpha mining in the realm of quantitative investment, developing a new interactive alpha mining system framework, Alpha-GPT. This system is centered on iterative Human-AI interaction based on large language models, introducing a Human-in-the-Loop approach to alpha discovery. In this paper, we present the next-generation Alpha-GPT 2.0 \footnote{Draft. Work in progress}, a quantitative investment framework that further encompasses crucial modeling and analysis phases in quantitative investment. This framework emphasizes the iterative, interactive research between humans and AI, embodying a Human-in-the-Loop strategy throughout the entire quantitative investment pipeline. By assimilating the insights of human researchers into the systematic alpha research process, we effectively leverage the Human-in-the-Loop approach, enhancing the efficiency and precision of quantitative investment research.

==> tex/experiment.tex <==
\tableAfterGP
\figureKlineComp
\tableOperators
\figureBacktestCurve
\figureAlphaExp
\section{Experiments}
We conduct experiments on Alpha-GPT with the goal of verifying the following research questions (RQ):
\begin{itemize}[leftmargin=*]
    \item \textbf{RQ1}: Can Alpha-GPT generate expressions that are consistent with the input trading ideas?
    \item \textbf{RQ2}: How effective is the algorithmic alpha mining layer in enhancing the seed alphas from LLM?
    \item \textbf{RQ3}: Can users effectively interact with Alpha-GPT to guide the mining process?
    \item \textbf{RQ4}: Can Alpha-GPT successfully explain the trading ideas behind alpha expressions?
\end{itemize}


\subsection{Experimental Setup}
The specifications of Alpha-GPT and other relevant information about our experiments include:

\textbf{Data and operators:} We use inter-day volume-price data of stock markets from US and China. This data includes the basic candlestick chart data (OHLCV), volume-weighted average price (VWAP), and sector data. We also include 19 basic operators implemented in \cite{guo_hxpy_2023} including time-series operations, cross-sectional operations, group-wise operations and basic element-wise operations, as shown in Table \ref{tab:operator}.

\textbf{Knowledge Library:} We construct the knowledge library based on the alphas proposed in \cite{kakushadze_101_2016}. For each alpha, we first decompose it into sub-expressions and explain them. Then we explain the combination of these sub-expressions to form the whole trading idea. Document embeddings are indexed via Faiss\footnote{https://github.com/facebookresearch/faiss}. Note that we only employed external memory when generating alphas for trading ideas that align well with those in \cite{kakushadze_101_2016}.

\textbf{LLM and Adapter:} For natural language interaction, we use OpenAI's chat completion API with ``gpt-3.5-turbo-16k-0613'' model base. For the embedding model used in knowledge retrieval, we use OpenAI's ``text-ada-embedding-002'' API with embedding dimension of 1536. The LLM generates a batch of alphas at a time, and will be asked to correct alphas with syntax or semantic errors.

\textbf{Alpha searching and evaluation:} Alphas are searched by the genetic programming model with a fitness score defined by the Information Coefficient (IC). We evaluate the performance of those alphas on out-of-sample criteria such as IC, annual return, Sharpe ratio, etc.


\subsection{Idea-Formula Consistency}
We first demonstrate that Alpha-GPT can generate formulaic alphas that are consistent with the user's given trading idea (\textbf{RQ1}). 
We come up with 3 different trading ideas from technical analysis. The trading ideas are combined with natural language descriptions to form Alpha-GPT inputs.
Figure \ref{fig:kline_vis} illustrates the generated alpha expressions based on given trading ideas and their correspondence to the patterns in the candlestick chart. The candlestick chart is plotted from the weekly data of the S\&P500 index from 2020 to 2023.

The first trading idea aims to capture golden cross patterns. The alpha value reflects the divergence between the fast and slow moving average curves. The second trading idea characterizes the breakout signals of Bollinger bands, and the corresponding alpha is a binary signal that gets activated when the upper bound is crossed. The third trading idea aims to capture three consecutive bullish movements on the candlestick chart, and the generated alpha successfully identified those patterns.
These examples demonstrate that the generated alphas correctly capture the trading ideas.

\subsection{Search Enhancement}
To verify that the alpha mining layer is capable of consistently enhancing the seeding alphas (\textbf{RQ2}), we compared the performance of both seed alpha and search-enhanced alpha for a given trading idea. The data used for computing alphas are from China's stock market.
Table \ref{tab:after_gp} shows the out-of-sample IC of alphas before and after search enhancement by the algorithmic alpha mining layer on 7 different trading ideas. We can see that search enhancement significantly improves the performance of Alpha-GPT and is critical in the Alpha-GPT workflow.

\subsection{Human-AI Interaction}
Figure \ref{fig:backtest_curve} illustrates the backtest curve of the alpha generated throughout the human-AI interaction. The backtest is conducted on US stock data from 2012 to 2021. The initial trading idea is to characterize the long-short imbalance. After several rounds of search enhancement and user interaction, the backtest performance of the resulting alphas significantly improved. More details about these interactions are present in the UI example in Figure \ref{fig:UI}.

\subsection{Alpha Explanation}
Figure \ref{fig:alphaexp} presents examples of alpha expressions generated by Alpha-GPT based on given trading ideas, and the corresponding natural language explanations of these alphas also generated by Alpha-GPT. From these examples we can see that Alpha-GPT can provide appropriate explanations of the generated alphas, relieving the burden of human researchers to interpret these expressions by themselves. 


==> tex/related.tex <==
\section{Related Work}
A lot of algorithms have been studied for formulaic alpha mining. Examples include Monte Carlo random search, Markov-chain Monte Carlo \cite{jin_bayesian_2020}, genetic programming \cite{cui_alphaevolve_2021} and their variants \cite{zhang_autoalpha_2020}, and reinforcement learning \cite{yu_generating_2023}.
% Besides, alpha performance and diversity can be used to guide the search progress, enabling the application of genetic programming \cite{zhang_autoalpha_2020, cui_alphaevolve_2021} to alpha mining.
% Moreover, in \cite{yu_generating_2023} deep neural networks are directly employed to generate alpha expressions in an autoregressive way, where reinforcement learning is applied for model training.
However, these methods all require the user to directly define the algorithmic configurations, providing limited interactivity compared with Alpha-GPT.
Meanwhile, LLMs such as GPT \cite{brown_language_2020} have demonstrated emergent abilities \cite{wei_emergent_2022} and achieved superior performance on various tasks.
% This paper demonstrates that we can leverage these abilities to 
Besides, LLMs have also shown great reasoning \cite{wei_chain--thought_2022, yao_tree_2023} and planning capabilities \cite{yao_react_2022}.
% Specifically, by parsing LLM outputs from natural language into structured data, we can enable LLMs to take specific actions or follow our instructions.
In this way, an LLM can be regarded as a core thinking module and be integrated with various peripheral tools \cite{schick_toolformer_2023} to form intelligent LLM-powered agents \cite{weng_llm_2023}.

\section{Conclusion and Future Work}
In this paper, we propose a new paradigm and a new system for alpha mining by leveraging the power of large language models. Further study on prompt engineering, LLM fine-tuning, alpha search algorithms, and knowledge library construction can be conducted to improve the capability of this system.


==> tex/sysarch.tex <==

\section{System Architecture }
Figure \ref{fig:arch} shows the system framework we proposed for Alpha-GPT 2.0. The system is a state-of-the-art framework designed to revolutionize the field of quantitative investment research. It is structured into three distinct layers: the Alpha Mining Layer, the Alpha Modeling Layer, and the Alpha Analysis Layer. Each of these layers plays a pivotal role in the overall functionality of the system, working in synergy to enhance the efficiency and effectiveness of quantitative investment research.

\subsection{Alpha Mining Layer}
\label{sec:sysarch_llm}
The Alpha Mining Layer is the foundation of the Alpha-GPT system, tasked with the crucial role of discovering and computing potential alpha factors. It starts with a comprehensive Data Ingestion Module that centralizes the collection of diverse market data, including stock prices, financial reports, and social media content. This aggregation of data is vital for providing a broad and detailed market perspective necessary for alpha discovery.

In the realm of alpha computation, the system employs advanced statistical and machine learning algorithms. This computation process is not only about identifying new alphas but also about refining and improving the efficiency of the alpha search process. The incorporation of Algorithm-Search Enhancement, utilizing techniques like genetic algorithms or deep learning, exemplifies the system's commitment to continuous improvement and adaptation to market changes.

Backtesting and evaluation form another critical aspect of this layer. Through rigorous historical performance analysis, the system assesses the validity and predictive power of identified alphas. This ensures that the alphas applied in trading strategies are both applicable and effective in real-world scenarios. Complementing this is the AlphaBase, a comprehensive repository that maintains a dynamic and updated database of validated alpha factors, enabling quick access for various investment strategies.

\subsection{Alpha Modeling Layer}
\label{sec:arch_compiler}
At the heart of Alpha-GPT lies the Alpha Modeling Layer, where the magic of model construction and optimization happens. This layer is pivotal in translating the identified alphas into actionable investment strategies. Utilizing cutting-edge AutoML technologies, the Alpha Auto-Modeling module automates the construction and optimization of alpha models, significantly streamlining the model-building process.

The rapidity and flexibility of model validation are also crucial. The Rapid Model Validation module facilitates swift deployment and assessment of various model structures, enabling quick iterations and refinements. This is further enhanced by the Quant Model Zoo, a curated library of quantitative trading models that serves as a valuable resource for model selection and innovation.

A key feature of this layer is the focus on Alpha Selection and Scoring. Based on the performance and market response, the system effectively selects and scores alphas, ensuring the relevance and impact of the chosen factors. Furthermore, a Feature Engineering Toolkit is provided, offering advanced tools and techniques for refining model inputs, which is instrumental in improving the accuracy and predictive quality of the models.

\subsection{Alpha Analysis Layer}
The final layer, the Alpha Analysis Layer, is where comprehensive analysis and optimization of investment strategies occur. It starts with the Factor Attribution Analysis module, which dissects the contribution of individual alpha factors to the overall investment strategy. This analysis is crucial for understanding the effectiveness of different alphas and guiding strategic adjustments.

Risk management is an integral part of any investment strategy. The Risk Analysis Module in this layer assesses various risks associated with the strategies, including market, credit, and liquidity risks. By doing so, it plays an essential role in safeguarding the investment portfolio.

The Portfolio Analysis \& Optimization module further enhances the system's capability by analyzing and optimizing the structure and performance of investment portfolios. This ensures that the portfolios are not only robust but also aligned with the investment goals and market conditions.

In addition, the Alpha Analysis Layer features FIN-QA, a sophisticated module that leverages large language models to provide deep insights into market dynamics and fundamentals. Complementing this is the Market Sentiment Analysis module, which utilizes natural language processing techniques to gauge market sentiment trends from news and social media. This holistic approach to market analysis provides a comprehensive view, offering an edge in understanding and predicting market movements.

In conclusion, the Alpha-GPT system, through its multi-layered architecture, offers a comprehensive solution for the challenges faced in quantitative investment research. By integrating advanced AI with the expertise of human researchers across these layers, the system not only streamlines the investment research process but also significantly enhances its depth and breadth.



\begin{comment}
\subsubsection{Thought Decompiler}
\label{sec:sysarch_middle_llm}

\algorithmRespParse     % see figures.tex

There is a significant gap between LLM responses and the desired output structure in alpha mining. Specifically, the gaps can be summarized as challenges from the following perspectives:
\begin{itemize}[leftmargin=*]
    \item \textbf{Nature language to structured data}: We need to convert LLM response from natural language to structured data. For each LLM response message, we need to extract a list of expression blocks from their raw outputs. And each expression block follows a certain organization style such as its short name, expression, and a paragraph of natural language description.
    \item \textbf{Token size limit}: Since most state-of-the-art LLMs apply a Transformer-based architecture with self-attention mechanisms, limits on the input sequence length (number of tokens) is usually a very common concern. In this way, both inputs and outputs of LLMs have an upper bound for their lengths. This may cause two issues: 1). We cannot keep sending full conversation history to LLMs since it will exceed the input token size limit. 2). The size of a single LLM response is limited, meaning that we can only get a limited number of expressions per message.

\end{itemize}

To address these issues, we propose an iterative LLM reasoning procedure (Algorithm \ref{alg:llm_reasoning}). We apply a parser based on regular expressions to parse LLM outputs. For each LLM-generated alpha, we validate its correctness both syntactically and semantically. We adopt an abstract syntax tree parser for syntax checking, and for semantic correctness, we evaluate this expression with mock data and runtime context to capture any exceptions being thrown out.

In practice, the proportion of correct alphas might be low (only 4 out of 10 alphas generated per round), making the alpha generation process inefficient. Meanwhile, since the conversation history is appended to LLM inputs, these incorrect expressions may also affect the generation process that follows. Hence, we apply an iterative correcting procedure where we prompt the LLM to re-generate incorrect alphas. 
Moreover, to address the problem of exceeded token size limit, at each round we dynamically check if the token size limit is exceeded, and if so, the input message will be truncated and reorganized to reduce the number of tokens. 

\subsubsection{Knowledge Library}
\label{sec:sysarch_middle_memory}

As mentioned in Section \ref{sec:arch_compiler}, few-shot in-context learning requires an external memory that supports efficient retrieval of demonstrations relevant to trading ideas. In Alpha-GPT, we design a protocol for organizing contents from across multiple sources. These range from an existing collection of alpha expressions to financial literature. When the user makes a request, the knowledge library encodes that query, and finds similar documents that it can incorporate into the prompt as examples. 

\subsection{Algorithmic Alpha Mining Layer}
This layer serves a search enhancement function in Alpha-GPT. Specifically, it implements an algorithmic alpha mining workflow by taking seed alphas and improving them with the received search commands and configurations from AlphaBot, and pushes the most appropriate alphas back to AlphaBot. It consists of four modules: the \textbf{algorithmic alpha search} module generates alpha candidates according to the commands from AlphaBot, qualified alphas are selected from these candidates using the \textbf{evaluation and backtesting} module, these alphas are further pruned according to a specific prediction target (e.g., contribution to the return of future 10 days) in the \textbf{alpha selection} module, and the final alphas are ``one-click'' deployed by the \textbf{alpha deployment} module to guarantee the smoothness and correctness of real-time computing during online trading.  

\subsubsection{Alpha Search Enhancement}
The most popular alpha search algorithm used in industry is genetic programming (GP), which starts from a number of alpha seeds and iteratively selects formulaic alphas expressed by trees using random crossing and mutation subtrees according to the fitness of a scoring function. However, GP currently suffers from three problems: 1) \textbf{Overfitting}, which is extremely dangerous for quantitative trading. This can be mitigated by strategies such as out-of-sample evaluation incorporated in GP iterations, fit regularization to reduce function complexity, and early stopping of iterations. These methods help ensure alphas generalize well beyond training data, improving their reliability. 2) \textbf{Loss of diversity} in alphas may result in the aggregation and accumulation of investment risk and increase the uncertainty of returns. Alpha diversification can be realized by enforcing more constraints in GP's iteration process, and it helps discover robust alpha factors that are resilient to changing market conditions. 3) \textbf{Invalid alphas} are easily generated by GP. For example, $log(0)$ and $\sqrt{-5}$, or a sum of two values with incompatible units (e.g, volume + close). Incorporating a rule base encompassing mathematical rules, unit consistency rule and financial domain-specific rules could regulate alpha expression generation.

\subsubsection{Evaluation and Backtesting}
The most straightforward method of evaluating alpha is through backtesting, which reveals the alpha's specific performance in an investment strategy. This process, however, introduces three significant challenges: 
1) \textbf{Introduction of future information}: information from a further point in time when backtesting could have disastrous consequences on result accuracy. To mitigate this, Timestamping is used to assign a time label to each piece of input data. This technique allows the backtesting system to more accurately replicate market conditions and validate test results, thereby enhancing the reliability of alpha evaluation. 2) \textbf{Estimation of transaction costs:} conventional coarse-grained backtesting cannot accurately measure transaction costs, which is crucial for short-term alphas. To solve this, we conduct a simulation-based \cite{amrouni_abides-gym_2021} backtest with trade matching rules using more detailed data, such as order book level data, for selected alphas. This enables us to model how transaction costs and market price impact alphas at a microstructure level. 3) \textbf {The computational cost}: the compute-power necessary for alpha mining is also significant, and we address this problem in the computation acceleration layer. 

\subsubsection{Alpha Selection}
The Alpha Selection module furthers the selection process in the following ways:
1) \textbf{Deduplication and Decorrelation:} new alphas need to be distinct from existing ones, but calculating pair-wise similarity between large amounts of alphas can be time-consuming. Algorithms like KD-Tree, Locality-Sensitive Hashing (LSH) \cite{gionis_similarity_1999}, or Approximate Nearest Neighbors (ANN) can swiftly determine each prospective alpha's maximum correlation with others in the pool. 
2) \textbf{Importance Scoring:} while an alpha's IC score and backtest may reflect individual performance, in real scenarios, multiple alphas are combined together in investment strategies, and these metrics do not accurately reflect how they perform in a larger set. A group of alphas with low IC scores may outperform a subset composed of the highest-scoring alphas. Thus, importance scoring techniques such as Shapley Additive exPlanations (SHAP) \cite{lundberg_unified_2017} and Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro_why_2016} measure this contribution and provide a comprehensive understanding of alphas in conjunction with one another.

\subsubsection{Alpha Deployment}
In this module, three key aspects need to be properly managed to guarantee the smooth and correct real-time computation during online trading: 1) \textbf{Dependency Management:} This involves maintaining and supervising all alpha-data inter-dependencies to ensure sequential computation and traceability of issues. 2) \textbf{Stream-Batch Unification:} Inconsistencies between live trading and historical backtesting of alphas are unacceptable. By adopting the Kappa Architecture, a unified real-time processing layer is maintained. Thus, all data is processed in the same manner, eliminating inconsistencies between batch and stream processing during alpha generation. 3) \textbf{Automatic Alpha Verification:} This is employed to validate all system-maintained alphas, monitor data quality, and identify discrepancies. This ongoing verification ensures the reliability, timeliness, and accuracy of the deployed alphas.

\subsection{Alpha Computation Acceleration Layer}
Alpha computation requires preprocessing financial data from various sources such as price-volume data, financial statement data, etc. Because of the computational overhead of processing high-frequency data such as orderbook level data, computational acceleration plays a key role. Also, in alpha mining, billions of alphas are calculated, making the speed of alpha calculations crucial for effectively exploring the alpha search space. Below we outline a few key computation acceleration techniques employed. \textbf{Streaming Algorithms:} particularly beneficial in performing rolling window computations on large time-series datasets. They incrementally update calculations with each new data point in the window, significantly optimizing computational efficiency and memory usage for these sliding-scale operations such as ts\textunderscore corr(rolling correlation of time-series data). 
\textbf{Vectorized Computation:} enables efficient financial data processing by eliminating explicit loops, leveraging hardware capabilities for concurrent processing, and optimizing memory management. \textbf{SIMD} (Single Instruction, Multiple Data) and \textbf{SIMT} (Single Instruction, Multiple Threads) \cite{hennessy_computer_2011}: allows simultaneous computations on multiple data points, fully exploiting hardware capabilities. \textbf{Memory Optimization}: pre-allocation of memory pool, layout optimization, and zero-copy, etc, are employed to minimize performance loss from discontinuous memory access and unnecessary memory allocation. \textbf{Data Partitioning}: Divides large-scale data into smaller, manageable chunks for independent processing. \textbf{Multithreading}: enables parallel computations on each partition using multiple threads. This approach significantly boosts computational speed when processing large financial datasets. \textbf{GPU Acceleration} \cite{nvidia_corporation_nvidia_2010}: employs CUDA cores for parallel processing, transforming CPU-bound operations into GPU-accelerated tasks and improves performance for data-intensive computations.
\end{comment}

==> tex/ui.tex <==
\section{User Interface of Alpha-GPT}
\label{sec:ui}
\figureUI
In Figure \ref{fig:UI} we introduce the web-based user interface (WebUI) of Alpha-GPT, which is composed of three main components: Session Manager, Dialog Box, and the Alpha Mining Dashboard.

\textbf{Dialog Box}: Users input their trading ideas and thoughts into the dialog box. In response, generated seed alphas, alpha searching progress, the final report of alpha mining, as well as the performance of the generated alphas, are all organized into system messages that provide comprehensive feedback. Users can then analyze the results and provide further direction for alpha mining, and this dialog continues until effective alphas are found.

\textbf{Mining Session Manager}: Alpha-GPT features a session-based user interface that stores past interaction history via the session manager. These sessions also serve to organize user-generated data, which can then be used to further enhance the system's performance.

\textbf{Alpha Mining Dashboard}: On the right half, the dashboard is used to display and analyze alpha mining results. It provides users with more detailed descriptions of the session. \textbf{Experiment Monitor} displays the alpha mining experiment progress and current system load as well as all historical alphas generated during a session. If a specific alpha is selected, its performances are plotted and visualized on the \textbf{Analytic Panel}. The available plotting features include a fitness curve across generations for genetic programming, a backtest curve for a single alpha, and other peripheral analyses such as IC distribution and Signal decay. Furthermore, \textbf{Alpha Dashboard} includes one-click storage and deployment, enabling further application and analysis downstream.

